Hybrid Low-Power Wide-Area Mesh Network for IoT Applications

The recent advancement of the Internet of Things (IoT) enables the possibility of data collection from diverse environments using IoT devices. However, despite the rapid advancement of low-power communication technologies, the deployment of IoT networks still faces many challenges. In this paper, we propose a hybrid, low-power, wide-area network (LPWAN) structure that can achieve wide-area communication coverage and low power consumption on IoT devices by utilizing both sub-GHz long-range radio and 2.4 GHz short-range radio. Specifically, we constructed a low-power mesh network with LoRa, a physical-layer standard that can provide long-range (kilometers) point-to-point communication using custom time-division multiple access (TDMA). Furthermore, we extended the capabilities of the mesh network by enabling ANT, an ultra-low-power, short-range communication protocol to satisfy data collection in dense device deployments. Third, we demonstrate the performance of the hybrid network with two real-world deployments at the Purdue University campus and at the university-owned farm. The results suggest that both networks have superior advantages in terms of cost, coverage, and power consumption vis-\`a-vis other IoT solutions, like LoRaWAN.

==> challenges.tex <==
\section{Design goal}

\label{sec:challenges}

\iffalse 
IoT deployment in the smart farming applications have several challenges to solve.  \textbf{First}, one device needs to be able to sample different types of information. It is impractical to install different sensors on various devices at the same place. \textbf{Second}, after the sensor data is sampled, how to reliably send the data to the central server. Failures may happen in the network due to different reasons such as environmental changes (coldness, raining, storms, etc) and communication failures. \textbf{Third}, how to trade off between the battery and communication cost as well as sensor cost. Communicating in a long range will require very high transmitting power while using several relaying nodes to route the data packet may cost less energy. As required by the first challenge, we want to have a variability of sensors on the same device but that will also cause more power consumption. Keep a low current while sensors are being sampled is necessary, especially we have multiple sensors on the same devices. \textbf{Fourth}, it is also important to monitor the battery life and replace any dead batteries in time. Given enough data points of battery levels, a practical approach is using some learning algorithms to predict the remaining life time of the device and notify developers when it drains to a low value. \textbf{Fifth}, after all the efforts, what radically important to enable the data analytics and the data visualization functions, which seems less interesting in research  but quite important in applications.  
\fi


%In conclusion, for any real world deployment, the theoretical wireless range and battery life is not reliable and normally must be much higher than the required specifications in order to maintain a normal operation and life span for the network.


%\subsection{Design goal}

To address the challenges mentioned in the introduction section, we designed a low-cost, low-power, robust, and light weight large area hybrid mesh network with following requirements:

\begin{itemize}
	\item Must be low-cost in system level, meaning not only hardware of the node is low-cost, the receiver (gateway) must be low-cost as well.
	\item Should be able to cover a large geographic area. For example, in our farming deployment, the network covers 2.2 $km^2$ of a farm and our campus deployment covers around 1.2 $km^2$ of Purdue campus.
	
	\item Has to be robust enough to survive the harsh environmental conditions and the network should able to handle node failures and recover from it.
	\item The deployment procedure for the IoT devices should not require any specific domain knowledge. Regular users should be able to simply install batteries to the IoT device and the device will work properly. 
	\item In addition to LoRa, the proposed network should also incorporate ultra-low power radio such as ANT to improve the performance and efficiency of the network in dense deployments.
	\item The proposed IoT device must be able to adopt to additional sensors.
\end{itemize}


%\begin{equation}
%d = ((\frac{c}{4\cdot\pi\cdot f})^{2} \cdot \frac{P_{tr} \cdot 2^{SF}}{SNR_{0} \cdot NF \cdot k \cdot T %\cdot BW})^{\frac{1}{n}}
%\end{equation}
%where $d$ is the range of LoRa, $P_{Tr}$ is the transmit power, $NF$ is the receiver architecture noise %figure, $k$ is the Kelvin constant, $T$ is the temperature and $BW$ is the bandwidth 




==> deployment.tex <==
\section{Deployment}
\label{sec:deployment}

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


==> network.tex <==
\section{Network Architecture}
\label{sec:network}

The IoT network architecture is important to provide the data reliability. A well-designed network can help reduce the effort of network recovery in the event of failures. To design the network architecture, two factors will determine the number of nodes as well as the topology of the network architecture. \textbf{First} is the device to device (D2D) communication range. D2D range determines how faraway the pairwise communication distance can be. Combined with the \textbf{second} factor which is the application area size and layout, they can determine how many nodes are needed in the application area. Once these two factors are decided, a network structure can be determined. Figure~\ref{fig:topologies} shows examples of the most common architectures for IoT network.

\begin{figure}[!t]
\centering
\includegraphics[width=1.0\linewidth]{pics/network_architectures.png}
\caption{Example of network architecture for IoT devices: (a) Star topology, with a central gateway connected to each nodes in the network; (b) Point-to-Multipoint Mesh Network, where each node acts as a router to extend the range of the network; (c) Zigbee, offers a simpler and faster communication using a coordinator node, router notes and end-devices; (d) DigiMesh, a more complex network but with a longer ranger where all nodes acts as router.}
\label{fig:topologies}
\end{figure}

\subsection{Star Network}
\label{subsec:network_star}

A typical network structure of IOT deployment is a star topology, where all nodes transmit their data to a central gateway. The star topology works fine if the distance between end-devices and gateway is within the reliable communication range of the protocol. However in the more complex IoT era today, it is possible that in some IoT applications, layout would be different in the line of sight between end device and gateway so that the end device cannot talk to the gateway because of the reduced D2D communication distance. For example, in a farmland when corns have been cut off, the D2D communication distance is much longer than the season when corns grow up. To adapt to such decrease in D2D communication distance due to environmental changes, developer has to install new gateways in those areas where some end devices are out of reach to the original gateways. This remedy will increase the infrastructure cost because installing a new gateway in a new place on the farmland will require additional power connectivity and Internet connectivity. 

\subsection{LoRaWAN}
\label{subsec:network_lorawan}

A common architecture for IoT devices to achieve long range distance is LoRaWAN, supported by the LoRa Alliance. LoRaWAN architecture~\cite{LoRaWAN} follows a star-of-stars topology, as shown in Figure~\ref{fig:lorawan}. In this network architecture, gateways relay messages between the end devices and a central network server. The communication between end devices is through LoRa, while the gateways are in an IP network within the central server. LoRaWAN is a MAC layer protocol built on top of LoRa as the link layer protocol, which enables long range transmission (around 10 kms on open areas) with low power consumption. The star topology works fine if the distance between end-device and gateway is within the reliable communication range of LoRa and the layout between an end device and a gateway is not dramatically changed. 

\begin{figure*}[!t]
\centering
\includegraphics[width=0.8\linewidth]{pics/lorawan_star}
\caption{The star topology of LoRaWAN network. Each end directly communications with LoRaWAN gateway and the LoRaWAN gateway sends collected data from end devices to the network server.}
\label{fig:lorawan}
\end{figure*}

\subsection{Mesh Network}
\label{subsec:network_mesh}

Since the star topology has limited scalability and adaptability in a dynamic IoT environment, mesh networks are used to expand the scalability. In a mesh network, end devices communicates between each other to transmit their data to a gateway. Overall, this network architecture has several advantage over a start network, but also adds complexity to the design of the network. First, a mesh network can significantly expand the communication coverage. This is very important in IoT farmland applications since the area is much bigger than the D2D distance of any low power transmission protocols. Second, a mesh network can provide the  redundancy of data transmission, increasing the communication reliability in the presence of transmission failures. A node in the mesh network usually has more than one neighbor. Therefore, when one neighbor is down, the other neighbors can be used to transmit the data to the gateways. Third, dynamics is provided in mesh network. When a new neighbor area is added to an existing mesh cluster, developers only need to physically install new nodes in neighbor area because they can join the existing cluster automatically in a dynamic mesh network. Fourth, end to end communication power is reduced. In a star topology where an end device is far away from the gateway, the end device has to increase the transmission power to reach the gateway while in mesh network, end device can use much lower transmission power since neighbor nodes are much closer than the gateway.

However, dynamic mesh network also comes with some challenges, such as the communication synchronization between end devices and the network configuration due to failures. Both scenarios increase the power consumption with respect to a traditional star topology. However, the overall advantages of mesh network clearly compensate the trade-offs.  
Since the communication is based in radio frequency, nodes in the mesh network have to agree on a common time window. During this time window a node acts as a sender while the neighbors should be prepare to receive the data. It is unwise and energy inefficient to keep the nodes in the receiving modes and waiting for data all the time. Furthermore, nodes in a mesh network need to be aware of the network topology to minimize the hops between nodes and gateways. For instance, it is unnecessary for several neighbor nodes to forward a common sender node's data. In these cases, a redundancy of two nodes should be enough to achieve a reliable communication. 

% Existing specification for IoT mesh networks include: \textit{DigiMesh}, \textit{Zigbee}...
% \edgardo{Explain briefly some mesh specifications used for IoT devices, such as DigiMesh, Zigbee.}
% \heng{Maybe unnecessary; I think a simple concept of Mesh has been enough. Our solution of ANT/LoRa mesh is more important.}

\subsection{ANT Low-Power Mesh Network}
\label{subsec:ANT_mesh}

ANT is a proprietary (but open access) multi-cast wireless sensor network technology by ANT Wireless. It defines a wireless communications protocol stack that enables hardware operating in the 2.4 GHz ISM band to communicate by establishing standard rules for co-existence, data representation, signaling, authentication, and error detection. It is conceptually similar to BLE(Bluetooth) low energy, but is oriented towards usage with sensors. With up to +4dbm TX power and -96 dBm sensitivity, our purposed testbed has a theoretical maximum range of approximately 1km (in line of sight) while maintaining a ultra low power consumption. This make ANT ideal for farm implementation XXX.

ANT shared channel is used to establish reliable bi-directional communication where a single ANT enabled device must receive, and possibly process, data from many nodes. In this scenario, multiple nodes(slaves) will share a single independent channel to communicate with the control node(master). This configuration is especially suited for applications in which a central node collects measurement data from a large number of sensors. ANT shared channels avoid the problem of contention among slave devices that can occur in standard ANT channels by using slave addressing. The master may give each slave device a unique address. This enables the polling of individual slaves to reliably retrieve measurement data. This creates a simple network structure with up to 65k slave devices sharing a single ANT channel. However, master devices in this configuration require to have knowledge of each slave device's address which is not usually the case.

ANT auto shared channel(ASC) is a extension to an ANT shared channel. It offers a simple method to dynamically and automatically add/remove slave devices to an ANT shared channel by adding an additional layer to register a new slave device with a shared channel master device. A ASC master device will have five operation states as follows:

\begin{itemize}[
    \setlength{\IEEElabelindent}{\dimexpr-\labelwidth-\labelsep}% Wrapping of text beyond first line of \item
    \setlength{\itemindent}{\dimexpr\labelwidth+\labelsep}% identation for each new \item
    \setlength{\listparindent}{\parindent}% Restore regular paragraph indentation
  ]
  \item Address available
  \item Handshaking
  \item Polling
  \item Sending command
\end{itemize}

When in Address available state, the ASC master is broadcasting whether it is able to take on more ASC Slaves. When a new slave wants to join the network, it will response to this broadcast to request a address. Once this request have been received by the ASC master device, handshaking process will be initiated which consists of a series of command and response messages passed between the master and slave devices. During this process, the nRF52832's serial number will used to identify the slave device to avoid conflict in assigning the address. After the assigned address has been confirmed by slave, master will register the slave device. Polling state indicates that master is requesting updates from each registered ASC Slave in order and ASC master can also send command to any specific slaves device in the network. This creates bi-directional mesh-like network with ultra low power consumption.

% \subsection{Adaptive Mesh Network}
% \label{subsec:network_adaptative}

% Even though the clear advantages that offers a mesh network over other network architectures, existing solutions are tied up with a specific protocol and do not have any awareness of changes in the deployment. Therefore, we have designed a dynamic mesh topology with both LoRa and ANT support. ANT has much lower power consumption than LoRa in data transmission and of course short communication range. However, in some applications sensor data are needed in a more restricted area (e.g. 1 $km^2$) and adding several LoRa nodes in such restricted area is a waste of LoRa's long reachability and is not energy efficient. Our mesh topology has the ability to dynamically switch between ANT and LoRa depending the application so that the D2D communication is conducted in an efficient way depending on the distance between device. Besides, our mesh network reduces the infrastructure cost because it only requires one gateway to provide the data collection capability in a large application area. Figure~\ref{fig:solution_architecture} is our architecture. In a restricted area (e.g. manufacture factory) where ANT mesh is enough to collect data and the installing an ANT gateway is convenient, we will only use ANT mesh to collect data. Whereas, in a large area (e.g. hundreds of square kilometers farmland), LoRa and ANT will provide the energy efficient approach to gather both fine grained environmental data as well as coarse grained environmental data. For example, a small plant space for soy beans can be satisfied by ANT mesh and its data will be routed through LoRa mesh to the LoRa gateway and upload to server. In such application, our custom board has the ability to switch LoRa transmission mode when enough amount of data needs to be uploaded to network server.

% \begin{figure*}[!ht]
% \centering
% \includegraphics[scale=0.40]{pics/mesh_architecture}
% \caption{Proposed Architecture. The nodes supports both LoRa and ANT protocols, but depending of the deployment or the scenario (e.g. communication range, power constraints) the protocol will be automatically selected to establish the communication between the nodes in the mesh.}
% \label{fig:solution_architecture}
% \end{figure*}

% An overview of the network in our deployment. 
% \begin{itemize}
% 	\item First, explain a simple configuration, start topology.
%     \item Then, move to the mesh topology. Highlight the advantage of the mesh topology, and the challenge to implement it. Static vs Dynamic architecture. How nodes communicate between each other? 
%     \item Include a figure of the overall architecture.
% \end{itemize}

\saurabh{Start with the simpler architecture, i.e., star and then move on to the mesh. Talk of the routing protocol to set up the mesh network.}

==> node.tex <==
\subsection{Sensing platform in Our Deployment}
\label{sec:node}

There are three main challenges when designing our platform for deployment: building a sufficiently light weight, low cost and energy efficient hardware capable of mass production, incorporating numerous subsystems to facilitate various applications (e.g.smart agriculture and smart city), and protecting the electronics from harsh environmental conditions.
\\

\subsubsection{ARM MCU and Wireless Radio Unit}

\hfill

A novel hardware platform was developed to support our network deployment by collaborating with HuWoMobility\cite{huwo} and utilizes their HMAA-1220 wireless transceiver module (Figure \ref{fig:sensor}). The HMAA-1120 wireless transceiver was powered by nRF52832 chip from Nordic Semiconductor\cite{nrf} and SX1262 LoRa transceiver from Semtech\cite{semtech}. nRF52832 features a low power 32-bit ARM Cortex-M4F processor with a built-in-radio that operates in the 2.4$GHz$ ISM band and support both ANT, BLE and Bluetooth 5 wireless protocol with up-to +4 $dBm$ transmit power. It is also equipped with 64$kB$ RAM and 512$kB$ of flash storage which can be used for storing data for in-node data analysis.

\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{pics/hardware}
\caption{huwo}
\label{fig:huwo}
\end{figure}

SX1262 from Semtech \cite{sx1262} is the new sub-GHz radio transceivers which are ideal for long range wireless applications. It supports both LoRa modulation for LPWAN applications and FSK modulation for legacy use cases. In addition, SX1262 also complies with the physical layer requirements of the LoRaWAN specification released by the LoRa Alliance\cite{lorawanspecification} and the continuous frequency coverage of SX1262 from 150 MHz to 960 MHz allows the support of all major sub-GHz ISM bands around the world. SX1262 was designed for long battery life with current consumption of 4.2$mA$ active receive mode and 600 $nA$ in sleep mode. With the highly efficient integrated power amplifiers, SX1262 can transmit up-to +22$dBm$ while having a high sensitivity down to -148$dBm$. Along with the co-channel rejection of 19$dB$ in LoRa mode and 88 dB blocking immunity at 1 MHz offset, SX1262 provides a maximum of 170$dB$ link budget which is ideal for long distance communication.

Figure \ref{fig:hardware} shows the printed circuit board(PCB) with it's packaging. The HMAA-1220 module was mounted on a "motherboard" with 4 LEDs and some pin-outs for connecting different "daughter board". This design choose allow us to extend the flexibility of our hardware platform to facilitate different applications.
\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{pics/board}
\caption{novel hardware}
\label{fig:hardware}
\end{figure}


\subsubsection{Sub-systems for Smart agriculture}
\hfill

As featured in Figure \ref{fig:hardware}, two daughter boards were designed for the smart agriculture application. We adopted three types of sensors for monitoring air, soil and water:

\begin{itemize}
  \item ECH2O 5TE [Fig. \ref{fig:sensor}(a)]: delivers temperature, measured by an on-board thermistor, along with accurate volumetric water content(VWC) by measuring the dielectric constant of the soil (or other media) using capacitance/frequency domain technology. Our system is capable of connecting 4 soil sensors for monitoring soil condition at four different levels.

  \item HDC2010[Fig. \ref{fig:sensor}(b)]: an integrated humidity and temperature sensor that provides high accuracy	measurements ($\pm$2 \% relative humidity, ±0.2$^{o}C$ ) with average supply current of 300$nA$.

  \item Nitrate sensor[Fig. \ref{fig:sensor}(c)]: The aim of these flexible nitrate sensors is to be used for detection of nitrate levels in the soil. The senors are fabricated by printing a silver ink onto a PET substrate. The sensing area is coated with an ion selective membrane, which is specific to nitrate ions, and the rest of the sensor is passivated with a silicon solution. The difference in potential between these nitrate sensitive sensors and a non-sensitive reference electrode is measured to determine the nitrate concentration in solution. The reference electrodes are fabricated in a similar fashion, with the main difference being that they lack the ion selective membrane and are instead passivated at the sensing area. 


  
\end{itemize}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.6\linewidth]{pics/sensor}
\caption{agriculture sensor}
\label{fig:sensor}
\end{figure}






